Phrase Retrieval Learns Passage Retrieval, Too

Dense retrieval methods have shown great promise over sparse retrieval methods in a range of NLP problems. Among them, dense phrase retrieval-the most fine-grained retrieval unit-is appealing because phrases can be directly used as the output for question answering and slot filling tasks. In this work, we follow the intuition that retrieving phrases naturally entails retrieving larger text blocks and study whether phrase retrieval can serve as the basis for coarse-level retrieval including passages and documents. We first observe that a dense phrase-retrieval system, without any retraining, already achieves better passage retrieval accuracy (+3-5% in top-5 accuracy) compared to passage retrievers, which also helps achieve superior end-to-end QA performance with fewer passages. Then, we provide an interpretation for why phrase-level supervision helps learn better fine-grained entailment compared to passage-level supervision, and also show that phrase retrieval can be improved to achieve competitive performance in document-retrieval tasks such as entity linking and knowledge-grounded dialogue. Finally, we demonstrate how phrase filtering and vector quantization can reduce the size of our index by 4-10x, making dense phrase retrieval a practical and versatile solution in multi-granularity retrieval.

==> sections/discussion.tex <==
%!TEX root = ../main.tex

\section{Discussion}
\label{sec:discussion}

\paragraph{Diverse retrieval}
\begin{itemize}
    \item prev works on retrieving diverse passages~\citep{min2021joint}
    
% \alex{Are we going to talk about the $\ell_{topic}$ and $\ell_{fine-grained}$ metrics here? Are you hesitant about including this analysis or just leaving this for later?}
% \jinhyuk{will add them in section 3.2!}
\end{itemize}

\paragraph{Multi-vector encoding}
\begin{itemize}
    \item how our model is related to multi-vector
\end{itemize}

==> sections/experiment.tex <==
%!TEX root = ../main.tex

\section{Experiments}
\label{sec:experiment}
We demonstrate the performance and versatility of phrase-based passage retrieval in two different settings: First, we examine whether the empirical benefits in retrieval observed in Section \ref{sec:prelim_exp} translate to gains in the full open-domain QA setting (\Cref{sec:openqa})
Second, we apply our system to document-level retrieval for entity-linking and knowledge-grounded dialogue in the KILT dataset \citep{petroni2021kilt} to show that it can be easily adapted to a new task and retrieval unit (\Cref{sec:kilt}).      

\begin{comment}
\subsection{Open-domain QA}\label{sec:openqa}
% While we have shown that DensePhrases can retrieve paragraphs in an equal setting to DPR, our system has some unique advantage: By using phrases as the most fine-grained retrieval unit, we can easily adapt the size of the context we would like to retrieve, without having to re-index the entire Wikipedia. In particular, this allows us to use much shorter passage, for example natural sentences.
Recently, \citet{izacard2020leveraging} have shown that a generative decoder can benefit from accessing a large quantity of (independently encoded) top-$k$ passages, achieving state-of-the-art performance on open-domain QA. However, processing up to 100 passages of 100 word length with a T5 model takes vast computational resources.%
\footnote{According to \citet{izacard2020leveraging}, it takes up to 425 GPU hours for training their largest model.}
In this case study, we ask the question if comparable performance can be achieved with smaller passages as the input, drastically reducing the computational requirements for this \textit{Fusion-in-Decoder} (FiD) approach.

% We emphasise that DPR cannot be used to retrieve sentences out-of-the-box, since there is no notion of where within a retrieved passage the answer lies.
% Note also that while our retrieved units are short, their phrase representations were encoded using the entire paragraph and thus are informed by the wider context. This also would not be possible in DPR.
\paragraph{Implementation Details}~
We evaluate each model on the two open-domain QA datasets used in \Cref{sec:prelim_exp}: Natural Questions~\citep{kwiatkowski2019natural} and TriviaQA~\citep{joshi2017triviaqa}.
For the experiments, we replace the retriever of FiD to DensePhrases-multi.
We use T5-base models to process up to top-50 passages, mainly due to the resource constraint.
DensePhrases can also retrieve sentences out-of-the-box by locating sentences that contain the phrases.
Hence, we train another T5-base model on top-100 sentences, which consumes much smaller GPU memory compared to using 100 passages.

\paragraph{Results}~
As shown in Table~\ref{tab:openqa-em}, using DensePhrases as a passage retriever achieves competitive performance with DPR + T5-base models.
Its better retrieval quality at top-$k$ indeed translates to better open-domain QA accuracy, achieving +6.4\% gain compared to DPR + T5-base when $k=5$.
To obtain comparable performance with using $k=100$ passages from DPR, DensePhrases only requires $k=25 \sim 50$ passages.
Although reading $k^*=100$ sentences requires much smaller memory than reading $k=100$ passages, its performance isn't as good as using passages, indicating that reading the passages is better than reading the sentences for the generative readers despite of its computational cost.

\end{comment}
% \jinhyuk{right granularity for T5 reader?}
% \danqi{Also address the memory concern?}



% To show how DensePhrases can be used to retrieve even larger granularity such as Wikipedia articles, we train and evaluate DensePhrases on the KILT~\citep{petroni2021kilt} benchmark which has multiple knowledge intensive language tasks.
% We also test our model on multi-answer QA tasks~\citep{min2021joint} to validate whether DensePhrases can retrieve a diverse set of passages.


\subsection{Coarse-grained Retrieval}\label{sec:kilt}
While DensePhrases has been directly used to retrieve phrases for open-domain QA and slot filling tasks~\citep{lee2021learning}, we further train DensePhrases to better retrieve coarse-grained retrieval units such as documents.
Specifically, we use entity linking and knowledge-grounded dialogue tasks from KILT~\citep{petroni2021kilt} where each model needs to provide a correct document in English Wikipedia.
We use document-level supervision as described in \Cref{sec:coarse} to train DensePhrases.

\paragraph{Results}~
In the last row of Table~\ref{tab:openqa}, we show the result of applying passage-level supervision during query-side fine-tuning.
Table~\ref{tab:kilt} shows the results on three entity linking tasks and a knowledge-grounded dialogue task.
\jinhyuk{results pending}

\input{tables/kilt}


\begin{comment}

\subsection{Efficient Phrase Retrieval}\label{sec:efficient-result}
% As discussed in \Cref{sec:multivec}, phrase-base passage retrieval is analogous to multi-vector encoding models where they also have multiple passage representations for each passage.
The multi-vector encoding models as well as ours are notoriously large since they contain multiple vector representations for every passage in the entire corpus.
% In this section, we experiment whether we can further compress our model by filtering phrases more aggresively and applying the efficient retrieval methods described in \Cref{sec:efficient}.
In Figure~\ref{fig:efficient}, we plot the changes in top-5 retrieval accuracy with respect to the size of the phrase index in DensePhrases.
By tuning the of phrase filtering properly, the number of vectors per each passage can be reduced without hurting the performance significantly.
The performance decreases with the smaller number of vectors per passage, which aligns with the findings of multi-vector encoding models~\citep{humeau2020polyencoders,luan2021sparse}.
While applying OPQ can reduce the size of the phrase index in DensePhrases from 320GB to 84GB, the top-5 retrieval accuracy also deteriorates a lot.
Applying quantization-aware query-side fine-tuning can recover the performance by mitigating the effect of quantization loss.

\begin{figure}[!t]
    \centering
     \includegraphics[scale=0.40]{figures/efficient}
     \caption{
     Top-$k$ accuracy on Natural Questions (dev) for different index sizes in DensePhrases.
     We can easily control the size of the phrase index of DensePhrases by tuning the filtering threshold.
     \jinhyuk{exact numbers will be changed}
     }
     \label{fig:efficient}
\end{figure}


\end{comment}

==> tables/comparison.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
    \begin{center}
    \centering
    \resizebox{2.0\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Retrieval Unit}} & \multicolumn{2}{c}{\textbf{Passage-level}} & \textbf{Phrase-level}
        & {\textbf{Storage}} & \multirow{2}{*}{\textbf{\#Q/sec}} \\
    % \cmidrule{4-5}
        & & Acc@1 & Acc@5 & Acc@1 & (GB)& \\
    \midrule
        % DrQA~\citep{chen2017reading} & Document & Bi-LSTM & 26 & 1.8, 0.6 & - & \\
        ORQA~\citep{lee2019latent} & 288 tokens & - & - & 33.3$^\dagger$ & 18 & 8.6 \\
        REALM$_\text{News}$~\citep{guu2020realm} & 288 tokens & - & - & 40.4$^\dagger$ & 18 & 8.4 \\
        DPR-multi~\citep{karpukhin2020dense}& 100 words & 44.4 & 67.1 & \textbf{41.5}$^\dagger$ & 76 & 0.9  \\
    \midrule
        DensePhrases~\citep{lee2020learning} & Phrase & - & - & 40.9 & 320 & 20.6 \\
        Phrase-based Passage Retrieval (Ours) & Phrase & \textbf{51.1} & \textbf{69.9} & 40.2 & 73 & 40.8 \\
        \tableindent + Phrase Filtering & Phrase & - & - & - & - & - \\
        % DenSPI~\citep{seo2019real} & \cmark & 1,200 & 2.9, 2.4 & 8.1 & 36.2\\
        % Passage Retrieval & DenSPI + Sparc~\citep{lee2020contextualized} & \cmark & 1,547 & 2.1, 1.7 & 14.5 & 40.7 \\
        
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        Comparison of different dense retrieval methods on the Natural Questions (open) test set. Passage-level Acc@$k$ is a proportion of questions whose predicted top-$k$ passages contain correct answers. We only report passage-level accuracies that are directly comparable to DPR, whose passages contain exactly 100 words each. Phrase-level Acc@$k$ is a proportion of questions whose predicted answer phrases are correct (same as the exact match in open-domain QA). $^\dagger$: obtained by running separate reader models (BERT-base) to extract answer phrases.
    }
    \label{tab:comparison}
\end{table*}



==> tables/contrasting_dpr_densephrases.tex <==
%!TEX root = ../main.tex

\begin{table*}[ht]
    \begin{center}
    \centering
    \resizebox{2.0\columnwidth}{!}{
    \begin{tabular}{p{0.1\linewidth}p{0.4\linewidth}p{0.4\linewidth}}
    \toprule
        &  \multicolumn{1}{c}{DPR} & \multicolumn{1}{c}{DensePhrases}  \\
    \midrule
        Training objectives & \multicolumn{1}{c}{\(
        \displaystyle
        -\log \frac{e^{f(p^+, q)}}{e^{f(p^+, q)} + \sum\limits_{p^- \in \mathcal{P}^-} e^{f(p^-, q)}}
        \)}
        & \multicolumn{1}{c}{\(
        \displaystyle
        -\log \frac{e^{f(s^+, q)}}{e^{f(s^+, q)} + \sum\limits_{s^- \in \mathcal{S}^-} e^{f(s^-, q)}}
        \)} \vspace{0.2cm} \\
        
    Encoder & BERT \citep{devlin2019bert} & SpanBERT \citep{joshi2020spanbert}  \\
    models & (\texttt{[CLS]} representations) & (concatenate phrase start and end repr.) \vspace{0.2cm} \\ 
    Positives & $p^+$ contains the answer to question $q$ & $s^+$ \textit{is} the answer to question $q$ \vspace{0.2cm} \\ 
    Negatives & $\mathcal{P}^-$ has {\color{princetonorange}in-batch} and {\color{cornellred}hard}$^\dagger$ negatives & $\mathcal{S}^-$ has {\color{princetonorange}in-batch} and {\color{darkmagenta}in-passage} negatives \\
    & ($^\dagger$mined by BM25 similarity with $q$)  \vspace{0.2cm} &  \\ 
    \hline
    Example & \multicolumn{2}{c}{$q = $ ``Which components of cells are physically connected by a gap junction?''} \\
    \hline 
    Positives & $p^+ = $ {``A gap junction may also be called a nexus or macula communicans...~They directly connect the cytoplasm of two cells, which allows various molecules...''} \vspace{0.2cm} & $s^+ = $ {``the cytoplasm''}  \\
    Negatives & $\mathcal{P}^- = \{$ {\color{cornellred}``it was found that chemicals could also be transported between cells through gap junctions.~Implicit or...''}, {\color{princetonorange}``Harry Allen (born October 12, 1966) is an American jazz tenor saxophonist...''}, ...$\}$ & 
    $\mathcal{S}^- = \{$ {\color{darkmagenta}``macula communicans''}, {\color{darkmagenta}``by modern definition''}, {\color{darkmagenta}``animal-cell types''}, {\color{darkmagenta}``when found in neurons or nerves''}, ..., {\color{princetonorange}``Jeremy Irons''}, {\color{princetonorange}``October 7, 2008''}, {\color{princetonorange}``15-yard line''}, {\color{princetonorange}``North Dakota''}, {\color{princetonorange}``ratify''}, ... $\}$ \\
    
    
    \hline
    \end{tabular}
    }
    \end{center}
    \caption{
        Contrasting the training objectives of DPR and DensePhrases.
    }
    \label{tab:contrasting}
\end{table*}


==> tables/efficient.tex <==
%!TEX root = ../main.tex


\begin{table}[t]
    \begin{center}
    \centering
    \resizebox{1.00\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
        \textbf{Model} & $\tau$ & \# vec / $p$ & Quant. & Size (GB) & Top-5 \\
    \midrule
        DensePhrases & 1.0 & 28.0 & SQ4 & 307 & - \\
        & 1.0 &  28.0 & OPQ96 & 69 & \textbf{69.0} \\
        & 2.0 &  17.9 & OPQ96 & 49 & 68.5 \\
        & 2.5 &  13.2 & OPQ96 & 40 & 68.1 \\
        & 3.0 &  8.8 & OPQ96 & 30 & 67.0\\
        & 3.5 &  5.1 & OPQ96 & {23} & 64.8 \\
        w/o QSFT & 1.0 & 28.0 & OPQ96 & 69 & 59.3\\
    \midrule
        DPR & - & 1  & None & 62 & 66.3 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        Top-5 passage retrieval accuracy on Natural Questions (dev) for different index sizes (GB) of DensePhrases.
        The index size of DensePhrases is controlled by the filtering threshold $\tau$.
        \#~vec~/~$p$: average number of saved vectors per passage. Quant.: quantization method. Size: vector index size.
        QSFT: quantization-aware query-side fine-tuning.
    }
    \label{tab:efficient}
\end{table}

\begin{figure}[!t]
    \includegraphics[scale=0.55]{figures/size_top5.pdf}
    \centering
    \caption{
        Top-5 passage retrieval accuracy on Natural Questions (dev) for different index sizes (GB) of DensePhrases.
        After applying OPQ~\citep{ge2013optimized}, the index size of DensePhrases is controlled by the filtering threshold $\tau$.
        \#~vec~/~$p$: average number of saved vectors per passage.
        QSFT: quantization-aware query-side fine-tuning.
    }\label{fig:efficient}\vspace{0.1cm}
\end{figure}


==> tables/mlm.tex <==
%!TEX root = ../main.tex

\begin{table}[ht]
    \begin{center}
    \centering
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
        {Model} & {STS-B} & {Avg. transfer} \\
    \midrule
        w/o MLM & \tf{87.38} & 82.96 \\
        w/ MLM \\
        \tableindent $\lambda=0.01$ & 86.98 & 83.45 \\
        \tableindent $\lambda=0.1$ & 86.84 & \tf{83.67} \\
        \tableindent $\lambda=1$ & 86.38 & 83.40\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        Ablation studies on masked language modleing.
    }
    \label{tab:mlm}
\end{table}


==> tables/multians.tex <==
\begin{table}[ht]
    \begin{center}
    \centering
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
        & \multicolumn{2}{c}{WebQSP} & & \multicolumn{1}{c}{AmbigQA} \\
        \cmidrule{2-3} \cmidrule{5-5}
        {Model} & {Dev} & {Test} && {Dev} \\
    \midrule
        \multicolumn{5}{c}{Trained on open-domain QA, $|p|$ = 100 words} \\
    \midrule
        DPR-multi & 43.6/24.4 & 44.8/23.1 && 49.1/33.8  \\
        % ... MRecall@10 & 47.7/25.2 & 47.7/23.0 && 54.1/38.3 \\
        DensePhrases-multi & 49.0/24.4 & && 43.1/28.1 \\
        % ... MRecall@10 & 49.8/22.8 & && 48.9/35.0 \\
    \midrule
        \multicolumn{5}{c}{Trained on WebQSP/AmbigQA, $|p|$ = 288 tokens} \\
    \midrule
        DPR$+$ &  \\
        DensePhrases & \\
        DensePhrases (+ passage) \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        Multi-answer open-domain QA results. We report MRecall@5 (all/multi-answers only). \jinhyuk{please detail the metric here @Alex}
    }
    \label{tab:multians}
\end{table}

